The XMM Cluster Survey: Exploring scaling relations and completeness of the Dark Energy Survey Year 3 redMaPPer cluster catalogue

We cross-match and compare characteristics of galaxy clusters identified in observations from two sky surveys using two completely different techniques. One sample is optically selected from the analysis of three years of Dark Energy Survey observations using the redMaPPer cluster detection algorithm. The second is X-ray selected from XMM observations analysed by the XMM Cluster Survey. The samples comprise a total area of 57.4 deg$^2$, bounded by the area of 4 contiguous XMM survey regions that overlap the DES footprint. We find that the X-ray selected sample is fully matched with entries in the redMaPPer catalogue, above $\lambda>$20 and within 0.1$< z <$0.9. Conversely, only 38\% of the redMaPPer catalogue is matched to an X-ray extended source. Next, using 120 optically clusters and 184 X-ray selected clusters, we investigate the form of the X-ray luminosity-temperature ($L_{X}-T_{X}$), luminosity-richness ($L_{X}-\lambda$) and temperature-richness ($T_{X}-\lambda$) scaling relations. We find that the fitted forms of the $L_{X}-T_{X}$ relations are consistent between the two selection methods and also with other studies in the literature. However, we find tentative evidence for a steepening of the slope of the relation for low richness systems in the X-ray selected sample. When considering the scaling of richness with X-ray properties, we again find consistency in the relations (i.e., $L_{X}-\lambda$ and $T_{X}-\lambda$) between the optical and X-ray selected samples. This is contrary to previous similar works that find a significant increase in the scatter of the luminosity scaling relation for X-ray selected samples compared to optically selected samples.

==> Sec6.1.tex <==
In this section, we investigate further why there are 291 redMaPPer clusters, with $\lambda>20$, undetected by the current X-ray observations (see Section \ref{sec:optical_sample}).  We do this by estimating the required {\em XMM} exposure time needed to achieve a minimum of 20 PN counts and a signal-to-noise (SNR) ratio of at least 3 (we note that, for this exploratory test, we are only assuming the use of the PN camera). These values were chosen as a cut-off because 85\% of redMaPPer clusters that were detected (i.e., the RM$_{\rm XCS}$ sample) have an SNR$>3$ (see Sect.~\ref{sec:snr_cut}) and 85\% had at least 20 PN counts.  To estimate the required exposure time, we use the following process: we start by estimating the X-ray luminosity based upon the redMaPPer measured $\lambda$, using the best-fit luminosity-richness relation given in Section~\ref{sec:x-ray_lambda_relations} (note for this test we ignore the uncertainties on the relation).  Using the redMaPPer determined redshift, this luminosity is converted into an expected flux.  Then, using the {\sc HEASARC} {\sc PIMMS} software and assuming an {\sc apec} model, we convert the flux into an {\em XMM} PN count rate.  For the input {\sc apec} model parameters, we assume the redMaPPer redshift, an nH estimated from \cite{2016A&A...594A.116H} at the position of the redMaPPer centre and a temperature estimated from the best fit temperature-richness relation given in Section~\ref{sec:x-ray_lambda_relations} (again using the input $\lambda$ values). To account for the background, we use the existing {\em XMM} observations and determine the background rate within an annulus 1.05-1.5$\,\times\,$r$_{500}$ centred on the redMaPPer centroid.  Values of $r_{500}$ were estimated assuming Equation~\ref{equ:rdelta}, with the temperature estimated again from the best-fit temperature-$\lambda$ relation. (We were unable to estimate a background for 15 clusters due to their proximity to the edge of the field-of-view.)  Finally, for the remaining 276 clusters where we could obtain a background estimate, we estimate the required minimum exposure time needed ``detect'' the cluster by fulfilling the above SNR and PN count criteria.

Using the method described above, we subtract the required exposure time calculated at the location of the cluster from the effective exposure time of the actual {\em XMM} observation used in the analysis (assuming an average exposure within the r$_{500}$ region).  Figure~\ref{fig:completeness_comparison.png} shows the distribution of these time differences, with red bars indicating clusters with observations that should be long enough to detect clusters (given the criteria above and the best fit luminosity-$\lambda$ relation); green bars indicate those clusters with observations that were not long enough to detect the respective clusters. For example, if an estimated exposure time of 15~ks is required to exceed an SNR$>3$ and detect 20 PN counts, but the existing exposure time of the XMM observation at that location was only 10~ks, it would appear in the +5ks bar (as a green bar in the distribution). Based upon this analysis, there are 118 clusters ($\approx$43\%) in Figure~\ref{fig:completeness_comparison.png} where the actual observation exposure times are not sufficient to fulfil our SNR and PN counts criteria at the location of the observed redMaPPer cluster (i.e. the green bars) and therefore we would not expect to detect them from our current observations.  Conversely, there are 158 clusters where the current exposure times should be sufficient to detect a cluster based on our SNR$>3$ and PN counts$>20$ criteria. Therefore, we need to explore the potential reasons why do we not detect these clusters. 

One reasonable explanation is that these undetected clusters are less luminous for their given richness than the luminosities estimated from the best-fit scaling relation. This is plausible given the detected clusters used to generate the best-fit Luminosity-$\lambda$ relation shows significant scatter around the mean.  As such, we re-ran the above analysis to determine the luminosity for each cluster at which the estimated exposure time needed to detect a minimum of 20 PN counts with an SNR $>3$ becomes greater than the current effective exposure time (i.e. the luminosity at which the cluster would become a green bar on the histogram in Figure~\ref{fig:completeness_comparison.png}).  To do this, we iteratively reduce the luminosity of the cluster from the value inferred from the best-fit Luminosity-$\lambda$ scaling relation and, at each step, calculate the required exposure time needed to detect a minimum of 20 PN counts with an SNR$>3$.  We continue this iteration until the luminosity reaches a level whereby the required exposure time to detect the cluster becomes greater than the actual effective exposure time.  This minimum luminosity detection limit for each cluster is displayed as a red point with a downward error on the original Luminosity-$\lambda$ scaling relation plot from Section~\ref{sec:x-ray_lambda_relations}, shown in Figure~\ref{fig:Lum_Lam_with_undetected}.  Similarly, we also consider the 118 clusters that could not have been detected during the analysis given their required exposure times were greater than their actual exposure times.  Here, we iteratively increase their luminosity until, again, the required time falls below the actual time.  These are also shown on Figure~\ref{fig:Lum_Lam_with_undetected} as green points.  As shown in Figure~\ref{fig:Lum_Lam_with_undetected}, there is one cluster that sits below the 3$\sigma$ scatter band.  On visual inspection, this cluster is classified as a point source by {\sc XAPA}, although the X-ray emission appears to be extended.  The cluster falls very close to a PN chip gap and visually has a peaked emission profile, possibly leading to the point source classification by {\sc XAPA}.  

Using the method outlined above, it is plausible that the 158 ``detectable'' redMaPPer clusters have luminosities that are lower than those expected from the best-fit scaling relation but still within the 3$\sigma$ scatter. It is worth noting that the results of this extra analysis are qualitatively consistent with the upper limits calculated in Section~\ref{sec:UL}. It should also be noted that we cannot rule out the possibility that the redMaPPer richness values may be overestimated (which would imply a higher X-ray luminosity for a cluster) rather than the luminosities being overestimated as assumed above.  It is clear that deeper X-ray data is needed for a complete sample of clusters (including the current non-detections), along with a well understood selection function, to truly understand both the completeness and properties of redMaPPer selected clusters.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{ReqExp_output_min20_final.pdf}
    \caption{Histogram showing the distribution of how many extra seconds of exposure time would be required to detect a minimum of 20 PN counts with a SNR$>3$ for the 276 redMaPPer clusters with a retrieved background estimate that are not confirmed by X-ray (see Sect.~\ref{sec:contamination}). Red bars to the left of zero indicate the 158 clusters with a current effective exposure time that are sufficiently long to detect a minimum of 20 PN counts with a SNR$>3$ assuming our best-fit Luminosity-$\lambda$ scaling relation and background estimates.  Green bars to the right show the extra time in ks that would be required to fulfil the same criteria for the remaining 118 clusters based on our best-fit scaling relations and with background estimates taken from the respective {\em XMM} observation.}
    \label{fig:completeness_comparison.png}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{L52_undetected_min__production20_upper.pdf}
    \caption{$L^{r500}_{X,52}-\lambda$ relation for the RM$_{\rm scaling}$ sample in blue.  Red points highlight undetected clusters in our sample, and the minimum luminosity at which the estimated required exposure time for a detection (assuming an SNR$>3$ and PN counts $>$20, see Sect.~\ref{sec:contamination}) exceeds the current effective exposure time.  Green point highlight undetected cluster, and the minimum luminosity values in order for the required exposure time for a detection (again assuming SNR$>3$ and PN counts $>$20) to fall below the current effective exposure time for those clusters (where the exposure time of the observation was insufficient for a detection).}
    \label{fig:Lum_Lam_with_undetected}
\end{figure}


==> binning.tex <==

\subsubsection{Binning}

For the XCS\textsubscript{scaling} $L^{r500}_{X,bol}$-$T_{X}$ relation (Figure \ref{fig:LT_scaling_relations}), we note that there is one cluster that sits outside (including error bars) the $3\sigma$ residual scatter (at $T_{X}$=0.99~keV, E(z)$^{-1} L^{r500}_{X,bol}$=0.6$\times$10$^{44}$~erg~s$^{-1}$).  Through bootstrapping, we confirmed this data point, if included in the fit, is the principal contributor to a shallowing of the relation's slope.  Consulting the XXL catalogue \citep{refId0}, the published temperature for this cluster is $T_{X}$=2.04~keV, which moves the data point firmly into the $1\sigma$ channel (note the luminosity is consistent with our measured value).  A temperature of 2.04~keV was further validated using the software package \textbf{X}-ray \textbf{G}enerate and \textbf{A}nalyse \citep[XGA,][]{2022arXiv220201236T}.  All three analysis methods (XXL, XGA and the analysis presented in this work) use a different binning routine to group the spectral channels before {\sc xspec} fits the spectrum to a model.  We use Heasoft's {\sc ftgrouppha},  XXL uses Heasoft's {\sc grppha} and XGA uses SAS's {\sc grpspec} command.  In this particular cluster instance, the {\sc ftgrouppha} binning for the PN camera generates a much lower temperature than the other methods.  We will explore the effect of binning method in a future paper.
